SmartAvatar: Text- and Image-Guided Human Avatar Generation with VLM AI Agents

SmartAvatar is a vision-language-agent-driven framework for generating fully rigged, animation-ready 3D human avatars from a single photo or textual prompt. While diffusion-based methods have made progress in general 3D object generation, they continue to struggle with precise control over human identity, body shape, and animation readiness. In contrast, SmartAvatar leverages the commonsense reasoning capabilities of large vision-language models (VLMs) in combination with off-the-shelf parametric human generators to deliver high-quality, customizable avatars. A key innovation is an autonomous verification loop, where the agent renders draft avatars, evaluates facial similarity, anatomical plausibility, and prompt alignment, and iteratively adjusts generation parameters for convergence. This interactive, AI-guided refinement process promotes fine-grained control over both facial and body features, enabling users to iteratively refine their avatars via natural-language conversations. Unlike diffusion models that rely on static pre-trained datasets and offer limited flexibility, SmartAvatar brings users into the modeling loop and ensures continuous improvement through an LLM-driven procedural generation and verification system. The generated avatars are fully rigged and support pose manipulation with consistent identity and appearance, making them suitable for downstream animation and interactive applications. Quantitative benchmarks and user studies demonstrate that SmartAvatar outperforms recent text- and image-driven avatar generation systems in terms of reconstructed mesh quality, identity fidelity, attribute accuracy, and animation readiness, making it a versatile tool for realistic, customizable avatar creation on consumer-grade hardware.

==> sections/gptwriting.tex <==
\section{Method}
\label{sec:method}

\noindent\textbf{Overview}
SmartAvatar is an LLM-guided system for generating personalized 3D avatars from portrait images or natural language descriptions. The system relies on three specialized large language models: a \textit{descriptor} for semantic attribute extraction, a \textit{generator} for Python code synthesis in Blender, and a \textit{refiner} for iterative editing as illustrated in Figure~\ref{fig:pipeline}. This section describes the procedural pipeline, prompt design, feedback loop, and the system's support for both auto-verification and user-guided editing.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/CustomAvatar_pipeline.png}
    \caption{CustomAvatar pipeline: (1) descriptor LLM extracts facial attributes; (2) generator LLM produces Blender‐compatible Python code; (3) optional refiner LLM iterates code to improve likeness based on similarity feedback; (4) final avatar is rendered when similarity exceeds threshold or iteration limit is reached.}
    \label{fig:pipeline}
\end{figure}

\noindent\textbf{Input--Output Pipeline}
Given a single image \(I_{\mathrm{orig}}\), SmartAvatar generates a 3D-rendered avatar \(I_{\mathrm{rend}}\) through the following stages:
\begin{enumerate}
    \item The descriptor LLM \(f_{\mathrm{des}}\) analyzes \(I_{\mathrm{orig}}\) to extract a structured set of attributes (e.g., age range, gender presentation, facial features, hairstyle, accessories).
    \item The generator LLM \(f_{\mathrm{gen}}\) receives this description and emits executable Blender-compatible Python code to synthesize the avatar.
    \item The code is embedded in a Blender script template, establishing scene parameters such as camera position and lighting.
    \item A similarity score is computed between the rendered result and the input image using a face embedding model. If the likeness is insufficient, refinement begins.
\end{enumerate}

\noindent\textbf{Prompt Engineering and Chain-of-Thought (CoT) Planning}
Each LLM is primed with structured prompts that include:
\begin{itemize}
    \item A curated API reference to constrain generation within the Blender avatar API.
    \item A chain-of-thought reasoning framework that encourages step-wise planning: observe $\rightarrow$ plan $\rightarrow$ generate code.
\end{itemize}

For example, the generator LLM explicitly reasons through steps such as selecting base morphs, applying adjustments for clothing or hairstyle, and assigning appropriate materials. This decomposed reasoning reduces hallucinations and increases consistency, especially when translating vague input prompts like “a basketball player” into detailed 3D edits.

\noindent\textbf{Refinement via Auto-Verification}
To address common LLM challenges—high parameter dimensionality, lack of real-time feedback, and limited visual understanding—we introduce a similarity-guided feedback loop. A vision encoder \(F\) maps both the original image and rendered output to a shared embedding space. The cosine similarity
\[
s = \cos\bigl(F(I_{\mathrm{orig}}),\,F(I_{\mathrm{rend}})\bigr)
\]
serves as an automatic metric for resemblance. If \(s < \tau\) and the iteration count \(i < N_{\max}\), the refiner LLM \(f_{\mathrm{ref}}\) is triggered. It receives the prior code, the similarity score, and rendered results, and returns targeted code modifications (e.g., changing skin tone, adjusting jaw width).

This loop continues until \(s \geq \tau\) or the iteration cap is reached. The refined code replaces the prior version in the script template.

\noindent\textbf{LLM-Based Evaluation (Optional Mode)}
As an alternative to embedding-based comparison, the refiner can self-assess likeness by appending an evaluation instruction:
\begin{quote}
\texttt{"Compare these two images and assign a similarity rating between 0\% and 100\%. If no edits are needed, output exactly: \# NO\_CHANGES."}
\end{quote}
The loop halts if the LLM returns \# NO\_CHANGES or if its similarity estimate \(s_{\mathrm{LLM}} \geq \tau\). This LLM-evaluation mode is useful in domains where embedding models are unreliable due to non-photorealistic renders or stylization.

\noindent\textbf{Semantic Input Interpretation}
SmartAvatar supports both image and text-based prompts. For textual input, the descriptor LLM extracts high-level semantics such as “tall,” “smiling,” or “wears formal clothing,” and translates them into actionable attributes. For visual inputs, a vision-language model parses the portrait and infers descriptors like hairstyle, age group, and expression, which are then passed to the generator.

The prompt framework ensures that regardless of modality, all inputs are normalized into the same intermediate semantic representation before rendering.

\noindent\textbf{User-Driven Editing}
After auto-generation, users may interactively refine avatars by issuing natural language edits (e.g., “make the hair longer” or “change outfit to business casual”). These post-hoc edits reuse the CoT generation flow with a modified instruction prefix, while freezing all other scene parameters. The refiner LLM interprets these requests and emits delta updates in Python, allowing seamless, user-friendly customization.

\noindent\textbf{Animating the Avatar}
Finally, SmartAvatar integrates with MotionAgent~\cite{wu2024motionagent} to animate the generated 3D avatars. Users can describe desired motion (e.g., “walk and wave,” “jump backward”) via natural language. The MotionAgent system interprets these commands and synthesizes coherent animation clips, supporting multi-turn interaction and real-time refinement.

\noindent\textbf{LLM Configuration}
Each of the LLM components operates under a tailored role:
\begin{itemize}
    \item \textbf{Descriptor LLM} \(f_{\mathrm{des}}\): Lightweight prompt for attribute extraction from text or images.
    \item \textbf{Generator LLM} \(f_{\mathrm{gen}}\): Chain-of-Thought planning plus code-template generation for initial Python synthesis.
    \item \textbf{Refiner LLM} \(f_{\mathrm{ref}}\): Feedback-guided and similarity-informed code adjustment agent.
\end{itemize}
All LLMs reload the curated API reference and operate within a constrained code environment to ensure syntactic and semantic validity.
